Optimal Oblivious Subspace Embeddings with Near-optimal Sparsity

An oblivious subspace embedding is a random $m\times n$ matrix $\Pi$ such that, for any $d$-dimensional subspace, with high probability $\Pi$ preserves the norms of all vectors in that subspace within a $1\pm\epsilon$ factor. In this work, we give an oblivious subspace embedding with the optimal dimension $m=\Theta(d/\epsilon^2)$ that has a near-optimal sparsity of $\tilde O(1/\epsilon)$ non-zero entries per column of $\Pi$. This is the first result to nearly match the conjecture of Nelson and Nguyen [FOCS 2013] in terms of the best sparsity attainable by an optimal oblivious subspace embedding, improving on a prior bound of $\tilde O(1/\epsilon^6)$ non-zeros per column [Chenakkod et al., STOC 2024]. We further extend our approach to the non-oblivious setting, proposing a new family of Leverage Score Sparsified embeddings with Independent Columns, which yield faster runtimes for matrix approximation and regression tasks. In our analysis, we develop a new method which uses a decoupling argument together with the cumulant method for bounding the edge universality error of isotropic random matrices. To achieve near-optimal sparsity, we combine this general-purpose approach with new traces inequalities that leverage the specific structure of our subspace embedding construction.

==> response.tex <==
We thank the reviewers for their feedback and comments. We thank reviewer A for providing a simpler explanation for the necessity of $1/\varepsilon^2$ dependence for sparsity in the i.i.d. entries model for S, and for pointing out that the version of OSNAP we work with has already been formally defined in previous work. We shall incorporate both these remarks in the final version of our submission, if it gets accepted. Regarding reviewer B's concerns about the notation for moments of random variables, we wish to kindly point to Section A.1 where we clarify the notations used in the paper. To make it clearer, we will move this section to the main body of the paper and explain the definition of this notation again in the key steps where it is used. The reason to use this notation is that we follow the convention from [13] for denoting moments owing to the similarity in our approach and theirs. 

% Decision pending -  To make this choice of notation more prominent, we will move the paragraph in section A.1 to the main body of the paper.
